Bridging the Omics Divide: A Modular Relational Approach to Multi-Layer Biological Data Management

Background: Rapid growth of high-throughput molecular data demands systems for efficient retrieval, integration, and scalability across omics layers. Traditional file-based workflows hinder cross-modal analysis and reproducibility because of fragmented storage and ad-hoc querying. Few existing tools for genomic variation data prioritize modular multi-omics integration. We developed vcf2db, a sample-centric relational framework modeling each omics modality as a distinct but linkable component centered on biological samples. This study evaluates whether this design delivers competitive genomic retrieval while enabling extension to additional molecular layers. Results: We implemented a proof-of-concept genomic schema and ingestion pipeline for annotated VCF data using the European subset of the 1000 Genomes Project (502 samples, 25 million variants). We benchmarked it against three established VCF-oriented tools on seven retrieval tasks: coordinate filtering, annotation-driven queries, genotype extraction, and aggregation. Under controlled conditions, vcf2db performed strongly on selective queries, often outperforming other systems for coordinate and annotation filters, and remained usable for genotype retrieval. Aggregation-heavy tasks were less efficient, indicating optimization targets. We also validated modular extensibility by adding a synthetic transcriptomic layer without modifying genomic tables, linking layers via shared sample identifiers. Conclusion: vcf2db supports cross-layer retrieval directly as SQL queries anchored on shared sample identifiers, enabling integrated multi-omics access that is difficult with file-based approaches.

==> sections/01_introduction/tables/rwTab.tex <==
\begin{comment}
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\begin{table*}[ht]
\centering
\footnotesize
\caption{Literature Review of Genomic Data Management Approaches}
\label{tab:lit_review}
\begin{tabularx}{0.9\textwidth}{Y Y Y Y Y}
\toprule
\textbf{Study/Technology} & \textbf{Database Type} & \textbf{Key Features} & \textbf{Expandability} & \textbf{Availability} \\
\midrule
Janetzki et al. \cite{janetzki2015genome} & Relational & Compares in-memory (MonetDB) vs. disk-based (PostgreSQL) for VCF data & Supports integration of phenotypic and genomic data & Open-source \\
\midrule
Dorok et al. \cite{DBLP:conf/dexaw/DorokBS14} & Relational & Implements per-base storage schema with custom SQL aggregation function for efficient site-by-site variant calling & Supports on-demand variant calling with configurable parameters & Open-source \\
\midrule
VCFdbR \cite{koomar2020vcfdbr} & Relational \& file-based & Offers Table-GT and File-GT modes with database-friendly ``long format" genotype storage to support biobank-scale data & Integrates with R/Bioconductor ecosystem and dbplyr for efficient SQL queries & Open-source \\
\midrule
Cutevariant \cite{schutz2022cutevariant} & Relational & Combines GUI with VQL domain-specific language and customizable plugin architecture & Supports VCF data with numerous extension features (Bed intersection, set operations) & Open-source \\
\midrule
GEMINI \cite{gemini} & Relational & Integrates diverse genome annotations with compressed genotype arrays for efficient storage and querying & Supports built-in annotations, custom annotations, and inheritance pattern analysis & Open-source \\
\midrule
Schulz et al. \cite{DBLP:journals/jbi/SchulzNFDT16} & NoSQL & Compares relational vs. NoSQL for genomic data & Highly extensible for diverse data types & Experimental code available on GitHub \\
\midrule
VCF-Miner \cite{hart2016vcf} & NoSQL & GUI with sample grouping and custom annotation preservation & Supports all VCF variant types and non-diploid organisms & Open-source \\
\midrule
VCF-Server \cite{jiang2019vcf} & NoSQL & Web-based multi-user interface with annotation, filtering and centralized VCF management & Supports custom annotations and disease-specific variant collections & Open-source \\
\midrule
Abdullah et al. \cite{DBLP:journals/tlsdkcs/AbdullahA20} & NoSQL & Scalable framework with distributed in-memory computing and columnar storage & Designed for multi-omic data integration & Research prototype \\
\midrule
VCFtools \cite{danecek2011variant} & File-based & Perl API and C++ tools for VCF validation, filtering and population statistics & Limited to VCF format & Open-source \\
\midrule
VIVA \cite{tollefson2019viva} & File-based & Combines filtering, data extraction, and visualization in a single command with interactive visualizations & Limited to VCF format with phenotype integration & Open-source \\
\midrule
re-Searcher \cite{karabayev2021re} & File-based & GUI-based VCF processing with memory-efficient chunk processing and genotype format conversion & Limited to VCF data & Open-source \\
\midrule
BrowseVCF \cite{DBLP:journals/bib/SalatinoR17} & File-based & Memory-efficient selective indexing with Wormtable and keyword-based filtering & Support for any VCF source with multi-sample grouping & Open-source \\
\bottomrule
\end{tabularx}
\end{table*}
\end{comment}

\begin{center}
\hspace*{-3em} 
\begin{tabularx}{\textwidth}{
             p{0.10\textwidth} 
             p{0.10\textwidth} 
             p{0.40\textwidth}  % Wide
             p{0.40\textwidth}  % Wide
             p{0.10\textwidth}}
\caption{Literature Review of Genomic Data Management Approaches}\label{tab:lit_review}\\
\toprule
\textbf{Study} & \textbf{Database Type} & \textbf{Key Features} & \textbf{Expandability} & \textbf{Availability} \\
\midrule
\endfirsthead

\caption[]{Literature Review of Genomic Data Management Approaches (continued)}\\
\toprule
\textbf{Study} & \textbf{Database Type} & \textbf{Key Features} & \textbf{Expandability} & \textbf{Availability} \\
\midrule
\endhead

\midrule
\multicolumn{5}{r}{{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot

% Your table rows here...
Janetzki et al. \cite{janetzki2015genome} & Relational & Compares in-memory (MonetDB) vs. disk-based (PostgreSQL) for VCF data & Supports integration of phenotypic and genomic data & Open-source \\
\midrule
% ... rest of your rows
Dorok et al. \cite{DBLP:conf/dexaw/DorokBS14} & Relational & Implements per-base storage schema with custom SQL aggregation function for efficient site-by-site variant calling & Supports on-demand variant calling with configurable parameters & Open-source \\
\midrule
VCFdbR \cite{koomar2020vcfdbr} & Relational \& file-based & Offers Table-GT and File-GT modes with database-friendly ``long format" genotype storage to support biobank-scale data & Integrates with R/Bioconductor ecosystem and dbplyr for efficient SQL queries & Open-source \\
\midrule
Cutevariant \cite{schutz2022cutevariant} & Relational & Combines GUI with VQL domain-specific language and customizable plugin architecture & Supports VCF data with numerous extension features (Bed intersection, set operations) & Open-source \\
\midrule
GEMINI \cite{gemini} & Relational & Integrates diverse genome annotations with compressed genotype arrays for efficient storage and querying & Supports built-in annotations, custom annotations, and inheritance pattern analysis & Open-source \\
\midrule
Schulz et al. \cite{DBLP:journals/jbi/SchulzNFDT16} & NoSQL & Compares relational vs. NoSQL for genomic data & Highly extensible for diverse data types & Experimental code available on GitHub \\
\midrule
VCF-Miner \cite{hart2016vcf} & NoSQL & GUI with sample grouping and custom annotation preservation & Supports all VCF variant types and non-diploid organisms & Open-source \\
\midrule
VCF-Server \cite{jiang2019vcf} & NoSQL & Web-based multi-user interface with annotation, filtering and centralized VCF management & Supports custom annotations and disease-specific variant collections & Open-source \\
\midrule
Abdullah et al. \cite{DBLP:journals/tlsdkcs/AbdullahA20} & NoSQL & Scalable framework with distributed in-memory computing and columnar storage & Designed for multi-omic data integration & Research prototype \\
\midrule
VCFtools \cite{danecek2011variant} & File-based & Perl API and C++ tools for VCF validation, filtering and population statistics & Limited to VCF format & Open-source \\
\midrule
VIVA \cite{tollefson2019viva} & File-based & Combines filtering, data extraction, and visualization in a single command with interactive visualizations & Limited to VCF format with phenotype integration & Open-source \\
\midrule
re-Searcher \cite{karabayev2021re} & File-based & GUI-based VCF processing with memory-efficient chunk processing and genotype format conversion & Limited to VCF data & Open-source \\
\midrule
BrowseVCF \cite{DBLP:journals/bib/SalatinoR17} & File-based & Memory-efficient selective indexing with Wormtable and keyword-based filtering & Support for any VCF source with multi-sample grouping & Open-source \\
\bottomrule
\end{tabularx}
\end{center}

==> sections/04_Results/tables/bestPerfSolut.tex <==
\begin{table}[htbp]
\centering
\caption{Benchmark results for seven query workloads.}
\label{tab:benchmark}
\begin{tabular}{l l c c l l c}
\toprule
Query & \makecell{Workload \\ class} & \multicolumn{2}{c}{\texttt{vcf2db} mean (s)} & Best cold performer & Best warm performer & \makecell{\texttt{vcf2db} rank \\ cold/warm} \\
\cmidrule{3-4}
& & cold & warm & & \\
\midrule
Q1 & Lightweight retrieval & 0.116 & 0.050 & cutevariant, 0.013\,s & cutevariant, 0.004\,s & 2 / 2 \\
Q2 & Annotation-driven filtering & 0.192 & 0.097 & \texttt{vcf2db}, 0.192\,s & \texttt{vcf2db}, 0.097\,s & 1 / 1 \\
Q3 & Rare HIGH-impact filtering & 20.246 & 8.976 & \texttt{vcf2db}, 20.246\,s & cutevariant, 7.082\,s & 1 / 2 \\
Q4 & Genotype retrieval & 8.502 & 7.889 & cutevariant, 2.071\,s & cutevariant, 1.944\,s & 2 / 4 \\
Q5 & Multi-allelic variant query & 45.171 & 43.828 & VCFdbR-file, 28.160\,s & cutevariant, 6.609\,s & 2 / 4 \\
Q6 & Gene-level aggregation & 291.337 & 210.955 & VCFdbR-file, 66.226\,s & cutevariant, 49.753\,s & 3 / 4 \\
Q7 & Chromosome-level aggregation & 124.751 & 120.424 & VCFdbR-file, 62.068\,s & cutevariant, 4.990\,s & 3 / 4 \\
\bottomrule
\end{tabular}
\end{table}

==> sections/04_Results/tables/table1.tex <==
\begin{table}[htbp]
\centering
\caption{Full-dataset execution times under cold- and warm-cache conditions (seconds)}
\label{tab:full_dataset_runtimes}
\begin{tabular}{l c c c c c c c c c c}
\toprule
& \multicolumn{2}{c}{vcf2db} & \multicolumn{2}{c}{cutevariant} & \multicolumn{2}{c}{VCFdbR-table} & \multicolumn{2}{c}{VCFdbR-file} & \multicolumn{2}{c}{vcf-miner} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
Query & Cold & Warm & Cold & Warm & Cold & Warm & Cold & Warm & Cold & Warm \\
\midrule
Q1 & 0.116 & 0.050 & 0.013 & 0.004 & 71.565 & 2.010 & 15.309 & 2.516 & 58.191 & 14.465 \\
Q2 & 0.192 & 0.097 & 654.163 & 11.050 & 17.543 & 0.460 & 14.202 & 0.398 & 1160.895 & 545.243 \\
Q3 & 20.246 & 8.976 & 168.877 & 7.082 & 125.298 & 22.081 & 30.588 & 21.472 & 608.662 & 574.777 \\
Q4 & 8.502 & 7.889 & 2.071 & 1.944 & 73.378 & 3.647 & 27.798 & 11.895 & 11.409 & 3.051 \\
Q5 & 45.171 & 43.828 & 73.175 & 6.609 & 91.191 & 13.451 & 28.160 & 13.937 & 717.441 & 168.721 \\
Q6 & 316.387 & 210.955 & 740.904 & 49.753 & 136.938 & 57.030 & 66.226 & 57.644 & --- & --- \\
Q7 & 124.751 & 120.424 & 71.847 & 4.990 & 146.570 & 54.112 & 62.068 & 55.084 & 726.425 & 170.284 \\
\bottomrule
\end{tabular}
\footnotesize{--- indicates missing data (vcf-miner for Q6). All times rounded to three decimals.}
\end{table}

==> sections/04_Results/tables/table2.tex <==
\begin{table}[htbp]
\centering
\caption{Warm/cold execution time ratios across systems and queries}
\label{tab:warm_cold_ratios}
\begin{tabular}{l c c c c c}
\toprule
Query & vcf2db & cutevariant & VCFdbR-table & VCFdbR-file & vcf-miner \\
\midrule
Q1 & 0.43 & 0.32 & 0.03 & 0.16 & 0.25 \\
Q2 & 0.51 & 0.02 & 0.03 & 0.03 & 0.47 \\
Q3 & 0.44 & 0.04 & 0.18 & 0.70 & 0.94 \\
Q4 & 0.93 & 0.94 & 0.05 & 0.43 & 0.27 \\
Q5 & 0.97 & 0.09 & 0.15 & 0.49 & 0.24 \\
Q6 & 0.67 & 0.07 & 0.42 & 0.87 & --- \\
Q7 & 0.97 & 0.07 & 0.37 & 0.89 & 0.23 \\
\bottomrule
\end{tabular}
\footnotesize{Ratio = warm runtime / cold runtime. Values rounded to two decimals. --- indicates missing data (vcf-miner for Q6).}
\end{table}

==> sections/04_Results/tables/table3_cold_.tex <==
\begin{table}[htbp]
\centering
\caption{Cold-cache execution times across dataset fractions (seconds)}
\label{tab:cold_scalability}
\begin{tabular}{l l r r r r r}
\toprule
Query & Fraction (\%) & \multicolumn{1}{c}{vcf2db} & \multicolumn{1}{c}{cutevariant} & \multicolumn{1}{c}{VCFdbR-table} & \multicolumn{1}{c}{VCFdbR-file} & \multicolumn{1}{c}{vcf-miner} \\
\midrule
Q1 & 1   & 0.124 & 0.015 & 14.070 & 14.295 & 9.441 \\
   & 10  & 0.113 & 0.016 & 25.962 & 14.622 & 12.770 \\
   & 50  & 0.120 & 0.016 & 72.122 & 15.861 & 31.489 \\
   & 100 & 0.116 & 0.013 & 71.565 & 15.309 & 58.191 \\
\midrule
Q2 & 1   & 0.216 & 30.407 & 14.616 & 13.988 & 516.330 \\
   & 10  & 0.223 & 108.486 & 16.291 & 13.962 & 557.842 \\
   & 50  & 0.215 & 488.047 & 17.383 & 14.161 & 818.962 \\
   & 100 & 0.192 & 654.163 & 17.543 & 14.202 & 1160.895 \\
\midrule
Q3 & 1   & 21.196 & 9.690  & 30.713 & 30.251 & 136.181 \\
   & 10  & 21.776 & 31.049 & 42.144 & 30.131 & 189.826 \\
   & 50  & 21.486 & 119.236 & 115.840 & 30.855 & 397.308 \\
   & 100 & 20.246 & 168.877 & 125.298 & 30.588 & 608.662 \\
\midrule
Q4 & 1   & 0.269 & 0.078 & 14.094 & 22.998 & 1.915 \\
   & 10  & 1.983 & 0.310 & 26.216 & 24.680 & 2.593 \\
   & 50  & 4.249 & 1.123 & 73.087 & 26.416 & 6.307 \\
   & 100 & 8.502 & 2.071 & 73.378 & 27.798 & 11.409 \\
\midrule
Q5 & 1   & 46.045 & 70.765 & 25.846 & 25.355 & 174.237 \\
   & 10  & 45.410 & 75.091 & 39.788 & 27.900 & 209.040 \\
   & 50  & 44.597 & 72.233 & 91.455 & 28.828 & 416.872 \\
   & 100 & 45.171 & 73.175 & 91.191 & 28.160 & 717.441 \\
\midrule
Q6 & 1   & 310.172 & 63.498 & 66.627 & 66.341 & --- \\
   & 10  & 310.916 & 153.708 & 74.456 & 65.959 & --- \\
   & 50  & 316.608 & 554.703 & 122.542 & 66.341 & --- \\
   & 100 & 316.387 & 740.904 & 136.938 & 66.226 & --- \\
\midrule
Q7 & 1   & 138.019 & 70.886 & 68.571 & 61.135 & 171.061 \\
   & 10  & 129.855 & 74.158 & 74.435 & 61.131 & 208.039 \\
   & 50  & 122.749 & 73.273 & 117.309 & 61.451 & 420.574 \\
   & 100 & 124.751 & 71.847 & 146.570 & 62.068 & 726.425 \\
\bottomrule
\end{tabular}
\footnotesize{--- indicates missing data (vcf-miner for Q6). All times rounded to three decimals.}
\end{table}

==> sections/04_Results/tables/table3_warm_.tex <==
\begin{table}[htbp]
\centering
\caption{Warm-cache execution times across dataset fractions (seconds)}
\label{tab:warm_scalability}
\begin{tabular}{l l r r r r r}
\toprule
Query & Fraction (\%) & \multicolumn{1}{c}{vcf2db} & \multicolumn{1}{c}{cutevariant} & \multicolumn{1}{c}{VCFdbR-table} & \multicolumn{1}{c}{VCFdbR-file} & \multicolumn{1}{c}{vcf-miner} \\
\midrule
Q1 & 1   & 0.061 & 0.006 & 1.935 & 2.329 & 3.876 \\
   & 10  & 0.059 & 0.005 & 2.223 & 2.194 & 4.916 \\
   & 50  & 0.049 & 0.006 & 2.185 & 2.344 & 9.937 \\
   & 100 & 0.050 & 0.004 & 2.010 & 2.516 & 14.465 \\
\midrule
Q2 & 1   & 0.112 & 12.771 & 0.458 & 0.380 & 430.874 \\
   & 10  & 0.110 & 11.600 & 0.357 & 0.388 & 437.650 \\
   & 50  & 0.106 & 11.521 & 0.397 & 0.390 & 504.238 \\
   & 100 & 0.097 & 11.050 & 0.460 & 0.398 & 545.243 \\
\midrule
Q3 & 1   & 9.063 & 7.218 & 21.710 & 21.429 & 185.411 \\
   & 10  & 8.720 & 7.052 & 21.376 & 22.176 & 227.867 \\
   & 50  & 9.390 & 7.711 & 22.141 & 21.369 & 393.773 \\
   & 100 & 8.976 & 7.082 & 22.081 & 21.472 & 574.777 \\
\midrule
Q4 & 1   & 0.173 & 0.033 & 2.090 & 7.650 & 0.956 \\
   & 10  & 1.006 & 0.225 & 2.084 & 8.034 & 1.169 \\
   & 50  & 3.962 & 1.065 & 2.796 & 10.134 & 2.078 \\
   & 100 & 7.889 & 1.944 & 3.647 & 11.895 & 3.051 \\
\midrule
Q5 & 1   & 45.028 & 6.482 & 13.686 & 13.856 & 98.688 \\
   & 10  & 44.434 & 6.361 & 13.558 & 13.871 & 132.835 \\
   & 50  & 43.317 & 6.571 & 13.415 & 13.948 & 113.224 \\
   & 100 & 43.828 & 6.609 & 13.451 & 13.937 & 168.721 \\
\midrule
Q6 & 1   & 248.430 & 49.537 & 57.267 & 56.960 & --- \\
   & 10  & 242.069 & 50.869 & 56.973 & 57.304 & --- \\
   & 50  & 236.920 & 49.971 & 57.063 & 56.960 & --- \\
   & 100 & 210.955 & 49.753 & 57.030 & 57.644 & --- \\
\midrule
Q7 & 1   & 123.078 & 4.815 & 56.839 & 54.331 & 110.529 \\
   & 10  & 122.115 & 4.809 & 57.948 & 54.344 & 106.356 \\
   & 50  & 119.770 & 4.871 & 57.480 & 54.147 & 130.324 \\
   & 100 & 120.424 & 4.990 & 54.112 & 55.084 & 170.284 \\
\bottomrule
\end{tabular}
\footnotesize{--- indicates missing data (vcf-miner for Q6). All times rounded to three decimals.}
\end{table}
